High-Accuracy Ranging and Localization with Ultra-Wideband Communications for Energy-Constrained Devices

Ultra-wideband (UWB) communications have gained popularity in recent years for being able to provide distance measurements and localization with high accuracy, which can enhance the capabilities of devices in the Internet of Things (IoT). Since energy efficiency is of utmost concern in such applications, in this work we evaluate the power and energy consumption, distance measurements, and localization performance of two types of UWB physical interfaces (PHYs), which use either a low- or high-rate pulse repetition (LRP and HRP, respectively). The evaluation is done through measurements acquired in identical conditions, which is crucial in order to have a fair comparison between the devices. The LRP devices that we tested have the same ranging and localization performance, but ten times (10x) lower power consumption, 6x lower energy consumption per distance measurement, and at least 8x higher coverage than the HRP devices. Therefore, UWB LRP devices can offer high-accuracy ranging and localization even to ultra-low-power devices in the IoT. We performed measurements in typical LOS and NLOS scenarios and propose theoretical models for the distance errors obtained in these situations. The models can be used to simulate realistic building deployments and we illustrate such an example. This paper, therefore, provides a comprehensive overview of the energy demands, ranging characteristics, and localization performance of state-of-the-art UWB devices.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/power_consumption_backup.tex <==
\subsection{Power Consumption}
\label{ssec:power-consumption}

\begin{figure*}[ht!]
	\centering
	\subfloat{%
		\label{}%
		\includegraphics[width=0.6\linewidth]{dw_current_consumption_profile_legend.pdf}%
	}\\
	% Don't include the legend in the numbering
	\setcounter{subfigure}{0}
	%	\centering
	\subfloat[3db Access]{%
		\label{fig:3db-power}%
		\includegraphics[width=0.4\textwidth]{images/3db_power_consumption_profile_new.pdf}
	}\quad%
	\subfloat[Decawave]{%
		\label{fig:dw-power}%
		\includegraphics[width=0.4\textwidth]{images/dw_power_consumption_profile_new.pdf}
	}
	
	\caption{Power consumption of (a) 3db Access and (b) Decawave DWM1001 tags (initiators). The main states of the chipsets are deep sleep (not shown for 3db Access), idle, transmission (\texttt{TX}), and reception (\texttt{RX}). Additionally, the Decawave module has the wake-up state, a final \texttt{TX} message containing IoT data, and a waitig time between the \texttt{RX} message and the final \texttt{TX} message during which the device waits for messages from other anchors, if available. In our case, there was only one Decawave anchor in the network. The DWM1001 profile includes the power consumption of the DW1000 UWB chip and a BLE microprocessor.}
	\label{fig:power-consumption-profile}
\end{figure*}


We measured the current consumption of 3db and Decawave DWM1001 devices with a Keysight DC Power Analyzer. The 3db IC core was powered with \SI{1.25}{\volt} and the typical supply voltage of Decawave is \SI{3.3}{\volt}~\cite{dw1000_datasheet}. 

As noted in Section~\ref{sec:setup}, the Decawave DWM1001 module contains, besides the DW1000 UWB chip, a BLE microprocessor, and a motion detector. \textcolor{red}{Unfortunately, the Decawave MDEK1001 module allows for measuring the current consumption only of the DWM1001 module, so including the BLE microprocessor and the motion detector. To minimize the energy consumption of the additional components, we deactivated the motion detector. However, the device needs the BLE module to join the network so this component could not be turned off. Therefore, alongside the measured current consumption of the DWM1001 module, we will also present the typical power consumption of the DW1000 UWB chip from the device datasheet}~\cite{dw1000_datasheet}.

\figurename~\ref{fig:power-consumption-profile} shows the power consumption profiles of 3db and Decawave initiators. The power was computed using the measured current consumption and considering a typical input voltage of \SI{1.25}{\volt} for 3db Access and \SI{3.3}{\volt} for Decawave. 

\figurename~\ref{fig:3db-power} shows the operation of a 3db initiator. The device stays in the idle mode between consecutive distance measurements. Once every $T$ seconds, where $T$ is the transmission period, the device transmits a message, then goes into the receive mode, processes the response, and computes the distance to the other device.

\figurename~\ref{fig:dw-power} shows the ranging process of the Decawave initiator. The device was programmed to use the low power mode, so it stays in the deep sleep state between consecutive distance measurements. When the device wakes up from the deep sleep mode, it goes into the idle state, after which it transmits one message and waits for the response of the anchors. In our case, there was only one anchor in the network, so the device processes a single response. The device transmits a final message, most likely with IoT data (so not necessarily related to ranging or localization), after which it goes back into the deep sleep state. 3db devices also have the capacity to go into a deep sleep mode with an average current consumption of \SI{500}{\nano\ampere}. The deep sleep current consumption of the DW1000 is \SIrange{50}{100}{\nano\ampere}~\cite{dw1000_datasheet}.

We isolate the most important modes, namely the idle, transmit (\texttt{TX}), receive (\texttt{RX}), and deep sleep (only for DWM1001), and compute their average power consumption in \tablename~\ref{tab:power-meas-stats}. In \figurename~\ref{fig:power-consumption-profile}, the transition periods when going into a certain state are highlighted for better visibility. However, when computing the average power consumption we ignored the transition period and took into account only the time spent in a particular state. \textcolor{red}{\tablename~\ref{tab:power-meas-stats} also shows the average power consumption of the DW1000 UWB chip considering a typical current consumption of \SI{72}{\milli\ampere} in the \texttt{TX} mode, \SI{119}{\milli\ampere} in the \texttt{RX} mode, \SI{18}{\milli\ampere} in the idle mode, and \SI{100}{\nano\ampere} during the deep sleep.} 


\begin{table}[t!]
	\caption{The average power consumption of 3db and Decawave devices.}
	\centering
	\begin{threeparttable}
		\begin{tabular}{l
				S[table-format=3.1, round-mode=places, round-precision=1, table-column-width=1.1cm] % , table-column-width=2cm
				S[table-format=3.1, round-mode=places, round-precision=1, table-column-width=1.1cm] % , table-column-width=2cm
				S[table-format=3.1, round-mode=places, round-precision=1, table-column-width=1.1cm] % , table-column-width=2cm
				S[table-format=4.1, round-mode=places, round-precision=1, table-column-width=1.1cm] % , table-column-width=2cm
			}
			\toprule
			
			\multirow{2}{*}{}
			& \multicolumn{4}{c}{\makecell{Average power consumption\tnote{$\ddagger$}~ [\si{\milli\watt}]}}  \\ [1ex] \cline{2-5} \\ [-1.5ex]
			
			& \multicolumn{1}{c}{TX} 
			& \multicolumn{1}{c}{RX}
			& \multicolumn{1}{c}{Idle}
			& \multicolumn{1}{c}{Deep sleep}  \\
			
			\midrule
			
			3db Access
			& 20.7 & 40.7 & 6.6 & \multicolumn{1}{c}{$6.25 * 10^{-4}$\tnote{*}} \\
			
			DWM1001\tnote{$\dagger$}
			& 297.7 & 507.21 & 47.9 & 3.9 \\
			
			DW1000
			& 237.6\tnote{*} & 392.7\tnote{*} & 59.4\tnote{*} & \multicolumn{1}{c}{3.3 * $10^{-4}$\tnote{*}} \\
			
			\bottomrule
		\end{tabular}
		
		\begin{tablenotes}
			\item[$\ddagger$]{Considering an input voltage of \SI{1.25}{\volt} for 3db Access and \SI{3.3}{\volt} for Decawave.}
			\item[*]{Based on the device datasheet.}
			\item[$\dagger$]{Includes the UWB DW1000 chip and a Nordic Semiconductor nRF52832 BLE microprocessor.}
		\end{tablenotes}
	\end{threeparttable}
	
	\centering
	\label{tab:power-meas-stats}
\end{table}

\textcolor{red}{The measured average current consumption of the DWM1001 module was \SI{90.2}{\milli\ampere} in the \texttt{TX} mode, \SI{153}{\milli\ampere} in the \texttt{RX} mode, and \SI{14.5}{\milli\ampere} in the idle mode, which is in line with the expected values of \SI{81}{\milli\ampere}, \SI{150}{\milli\ampere}, and \SI{13}{\milli\ampere} in the respective modes from the DWM1001 datasheet~\cite{dwm1001_datasheet}. However, the measured deep sleep current consumption was more than $100$ times higher than expected: \SI{1.2}{\milli\ampere} instead of \SI{24}{\micro\ampere}. The deep sleep current consumption depends on the active peripheral components and is, in the best case about \SIrange{12}{15}{\micro\ampere} when only the RTC clock is active and the microcontroller is in the deep sleep mode~\cite{dwm1001_datasheet}. The power consumption of the DWM1001 is indeed higher than the expected power consumption of the DW1000 chip alone, so for the comparison with 3db devices we will rely on the datasheet power consumption of the DW1000 chip.}

Overall, the average power consumption of the 3db IC is \textcolor{red}{10 times lower} \hl{TODO Make sure this is the precise number} than the one of the Decawave IC. Note that the average power consumption of the DW1000 chip in the \textit{idle} mode is about $1.45$ times higher than the one of 3db devices in the \textit{receive} mode, also the most power-hungry state. So it seems that, indeed, the LRP interface can be more power-efficient than the HRP one.

The power consumption profile is a starting point for evaluating the energy consumption of an UWB-based localization system. A key challenge in a localization system is minimizing the energy consumption of the \textit{tag}, which is usually battery-powered. 
To avoid synchronizing the tag and the anchors, the tag can \textit{initiate} the message exchange and stay in the idle or sleep mode between rangings.
Using the SS-TWR implies, in this case, that the \textit{tag} estimates the distance (or the location). 

To illustrate the energy efficiency of a tag in a localization system, let us consider the most favorable scenario for each device, in which the tag is the initiator. We disregard the time spent in the idle mode, since it is subject to the desired location update rate and guard times, which can be chosen freely to a certain extent. We therefore compute the energy  consumption only when the device is in the \texttt{TX} or \texttt{RX} mode. The packet duration of the DW1000 chip in Mode 14 is \SI{287}{\micro\second} and the one of the 3db chip is \SI{400}{\micro\second}. Therefore, a Decawave tag will consume \SI{180}{\micro\joule} per SS-TWR during transmission and reception, while a 3db tag will consume \SI{28}{\micro\joule} (including the transition times), so $6.4$ times less energy. When placed in the long-range mode (for instance, mode 3), the packet duration of Decawave devices increases to \SI{3487}{\micro\second} which is about $10\times$ larger than that of 3db devices, causing them to consume at least than $100\times$ more energy~\cite{flueratoru2020energy}. The difference between these modes is the \textit{maximum range} at which the devices can communicate, so in the next section we will compare the range of 3db and Decawave devices.
